An Operator Product Expansion for Polygonal null Wilson Loops

We consider polygonal Wilson loops with null edges in conformal gauge theories. We derive an OPE-like expansion when several successive lines of the polygon are becoming aligned. The limit corresponds to a collinear, or multicollinear, limit and we explain the systematics of all the subleading corrections, going beyond the leading terms that were previously considered. These subleading corrections are governed by excitations of high spin operators, or excitations of a flux tube that goes between two Wilson lines. The discussion is valid for any conformal gauge theory, for any coupling and in any dimension. For N=4 super Yang Mills we check this expansion at strong coupling and at two loops at weak coupling . We also make predictions for the remainder function at higher loops. In the process, we also derived a new version for the TBA integral equations that determine the strong coupling answer and present the area as the associated Yang-Yang functional.

==> toc.tex <==
\noindent {1.} {Introduction} \leaderfill{1} \par 
\noindent {2.} { Symmetries } \leaderfill{4} \par 
\noindent \quad{2.1.} { The symmetries preserved by null lines and the square Wilson loop } \leaderfill{5} \par 
\noindent {3.} { The collinear operator product expansion } \leaderfill{8} \par 
\noindent \quad{3.1.} {A three parameter family of polygons} \leaderfill{8} \par 
\noindent \quad{3.2.} {States propagating in the expansion } \leaderfill{10} \par 
\noindent \quad{3.3.} {Taking care of violations of conformal symmetry: the remainder function} \leaderfill{14} \par 
\noindent \quad{3.4.} {Taking care of violations of conformal symmetry without using the $U(1)$ or one loop answer} \leaderfill{16} \par 
\noindent {4.} { Detailed checks for the hexagon } \leaderfill{18} \par 
\noindent \quad{4.1.} { Expansion of the hexagon at strong coupling } \leaderfill{18} \par 
\noindent \quad{4.2.} {Expansion of the hexagon at weak coupling } \leaderfill{19} \par 
\noindent {5.} {Higher order predictions} \leaderfill{22} \par 
\noindent {6.} {Conclusions} \leaderfill{22} \par 
\noindent {7.} {Acknowledgments} \leaderfill{23} \par 
\noindent Appendix {A.} {Describing the family of polygons in terms of momentum twistors} \leaderfill{23} \par 
\noindent Appendix {B.} {The hamiltonian picture and its analytic continuation} \leaderfill{24} \par 
\noindent \quad{\hbox {B.}1.} {Analytic continuation at strong coupling} \leaderfill{26} \par 
\noindent Appendix {C.} { Remarks on the dispersion relation } \leaderfill{29} \par 
\noindent \quad{\hbox {C.}1.} {Massive Goldstone particles } \leaderfill{30} \par 
\noindent Appendix {D.} {On the expansion for Wilson loops in the $U(1)$ theory} \leaderfill{31} \par 
\noindent Appendix {E.} {The modified TBA and Yang-Yang functional for $AdS_3$ null polygons} \leaderfill{32} \par 
\noindent \quad{\hbox {E.}1.} {Evaluating the OPE for general configurations in $AdS_3$} \leaderfill{37} \par 
\noindent Appendix {F.} {The modified TBA and Yang-Yang functional for $AdS_5 $ null polygons} \leaderfill{38} \par 
\noindent \quad{\hbox {F.}1.} {Explicit details for the hexagon} \leaderfill{39} \par 
\noindent \quad{\hbox {F.}2.} {Easy pieces of the hexagon} \leaderfill{44} \par 
\noindent \quad{\hbox {F.}3.} {Expanding the hexagon at strong coupling} \leaderfill{44} \par 

